Highly Scalable Task Grouping for Deep Multi-Task Learning in Prediction of Epigenetic Events

Deep neural networks trained for predicting cellular events from DNA sequence have become emerging tools to help elucidate the biological mechanism underlying the associations identified in genome-wide association studies. To enhance the training, multi-task learning (MTL) has been commonly exploited in previous works where trained networks were needed for multiple profiles differing in either event modality or cell type. All existing works adopted a simple MTL framework where all tasks share a single feature extraction network. Such a strategy even though effective to certain extent leads to substantial negative transfer, meaning the existence of large portion of tasks for which models obtained through MTL perform worse than those by single task learning. There have been methods developed to address such negative transfer in other domains, such as computer vision. However, these methods are generally difficult to scale up to handle large amount of tasks. In this paper, we propose a highly scalable task grouping framework to address negative transfer by only jointly training tasks that are potentially beneficial to each other. The proposed method exploits the network weights associated with task specific classification heads that can be cheaply obtained by one-time joint training of all tasks. Our results using a dataset consisting of 367 epigenetic profiles demonstrate the effectiveness of the proposed approach and its superiority over baseline methods.

==> BIBM paper 2022-082122/sections/related-work.tex <==

\section{Related work}

\subsection{Multi-task learning}

Basic idea of multi-task learning, and discussion on different ways of parameter sharing

Handle task interference

Working that utilize model weights in 

\subsection{Predicting functional genomic events}

Public research projects such as ENCODE \cite{feingold2004encode} and the Roadmap Epigenomics project \cite{kundaje2015integrative} with the aim of identifying functional elements in the human genome have collected a large number of epigenetic profiles including histone modifications(HM), transcription factor(TF) binding, and chromatin accessibility(CA) from a wide variety of cells. In recent years, deep multi-task learning models have achieved state-of-the-art performance for simultaneous prediction of a variety of epigenetic event profiles in different tissues \cite{zhou2015predicting, zhou2018deep, kelley2018sequential, kelley2020cross, avsec2021effective}. However, the task-relatedness among a large number of epigenetic event profiles has never been studied. In this paper, we developed groups of relevant tasks to benefit from each other in training a deep learning model.

Humans can transfer and share knowledge across various related fields when solving a specific task. Expanding such an effective paradigm to the area of artificial intelligence can potentially make advances in the performance of machine learning models. In recent years, there has been a growing interest in multi-task learning (MTL)\cite{caruana1997multitask, pratt1998learning}, which learns a shared representation among multiple related tasks at the same time. In contrast to single-task learning (STL), it can reduce the training and inference time, increase data efficiency, and improve generalization performance and prediction accuracy. The importance of MTL is in building models for tasks with limited data.

Hard and soft parameter sharing are the two most common techniques of performing MTL in deep neural networks \cite{ruder2017overview}. In hard parameter sharing, there is one model with shared hidden layers between all tasks except some of the output layers are task-specific. While soft parameter sharing is to have a separate task-specific model for each task and add the distance between model parameters to the joint objective function. Some work has been done on deciding what parameters to share across which tasks to improve the performance of MTL model in hard parameter sharing \cite{lu2017fully, sun2020adashare, vandenhende2019branched}.

The main goal in multi-task learning is to improve individual tasks by focusing on task relatedness, which is non-trivial since the tasks might be learned with different learning rates or tasks, some tasks may be dominated by other tasks' poor learning, or interference between tasks gradients in backward propagation can impact on the generalization of model. Some gradient-based techniques have been proposed to solve the gradient conflict between tasks which mostly compare gradients of each pair of tasks \cite{sener2018multi, chen2018gradnorm, yu2020gradient}.

Training a good MTL model can be more difficult when the number of tasks grows, and improper sharing of information across unrelated tasks may lead to negative transfer. Accordingly, finding groups of tasks that can benefit from training together in an MTL setting is a promising way to avoid negative transferring and train a more accurate model that can perform better than simply training all tasks together \cite{standley2020tasks, fifty2021efficiently, kang2011learning}. The problem of deciding which tasks should be trained together recently has been tackled by human experts or algorithmic. Some MTL modeling approaches capture relationships among tasks by assuming that the task relationships are not known beforehand and can be learned directly from the data \cite{kang2011learning, jacob2008clustered, zhang2012convex}.

In \cite{jacob2008clustered} tasks are assumed to be clustered and parameters of tasks within a cluster lie close to each other in $ \ell2 $ norm sense and learn shared features with convex optimization. In \cite{zhang2012convex} tasks are assumed to share a common yet latent feature representation and learn shared features with convex optimization. In \cite{kang2011learning} tasks are assumed to form disjoint groups and that the tasks within each group lie in a low-dimensional subspace. Within each group, tasks share the same feature representation, whose parameters are learned jointly with the group assignment matrix using an alternating minimization scheme. However, a total disjointness between groups might not be the ideal way, as the tasks might still share some features that are helpful for prediction.



==> BIBM paper 2022-082122/temp.tex <==
Multi-task learning (MTL) has been used successfully across all applications of machine learning, from natural language processing [Collobert and Weston, 2008] and speech recognition [Deng et al., 2013] to computer vision [Girshick, 2015] and drug discovery [Ramsundar et al., 2015].

In The function of TFs is to regulate expression of the correct number of genes in the body at the right time. TFs play important functions in many biological processes, such as gene transcription regulation, participation in developmental processes, and are closely related to many diseases. HM changes the binding environment of TFs to target sites by affecting the affinity between histone and DNA [9].

We assume that our data consists of $n$ “points” $x1,...,xn$ which can be arbitrary objects. We measure their pairwise similarities sij = s(xi,xj ) by some similarity function which is symmetric and nonnegative, and we denote the corresponding similarity matrix by $S = (s_{ij})_{i,j=1,...,n}$.

Given a dataset of $n p-dim$ points, $D = \{x_j\}^n_{j=1}$, the kmeans algorithm partitions the $n$ points into $k$ clusters, and represents each cluster by a center point. Let $C \in \mathbb{R}^{p×k}$ be a matrix whose columns comprise the $k$ cluster centers, i.e., $C = [c_1, c_2, \cdots , c_k]$. The k-means objective is to minimize the within-cluster squared distances:

==> sections/related-work.tex <==

\section{Related work}

\subsection{Multi-task learning}

Basic idea of multi-task learning, and discussion on different ways of parameter sharing

Handle task interference

Working that utilize model weights in 

\subsection{Predicting functional genomic events}

Public research projects such as ENCODE \cite{feingold2004encode} and the Roadmap Epigenomics project \cite{kundaje2015integrative} with the aim of identifying functional elements in the human genome have collected a large number of epigenetic profiles including histone modifications(HM), transcription factor(TF) binding, and chromatin accessibility(CA) from a wide variety of cells. In recent years, deep multi-task learning models have achieved state-of-the-art performance for simultaneous prediction of a variety of epigenetic event profiles in different tissues \cite{zhou2015predicting, zhou2018deep, kelley2018sequential, kelley2020cross, avsec2021effective}. However, the task-relatedness among a large number of epigenetic event profiles has never been studied. In this paper, we developed groups of relevant tasks to benefit from each other in training a deep learning model.

Humans can transfer and share knowledge across various related fields when solving a specific task. Expanding such an effective paradigm to the area of artificial intelligence can potentially make advances in the performance of machine learning models. In recent years, there has been a growing interest in multi-task learning (MTL)\cite{caruana1997multitask, pratt1998learning}, which learns a shared representation among multiple related tasks at the same time. In contrast to single-task learning (STL), it can reduce the training and inference time, increase data efficiency, and improve generalization performance and prediction accuracy. The importance of MTL is in building models for tasks with limited data.

Hard and soft parameter sharing are the two most common techniques of performing MTL in deep neural networks \cite{ruder2017overview}. In hard parameter sharing, there is one model with shared hidden layers between all tasks except some of the output layers are task-specific. While soft parameter sharing is to have a separate task-specific model for each task and add the distance between model parameters to the joint objective function. Some work has been done on deciding what parameters to share across which tasks to improve the performance of MTL model in hard parameter sharing \cite{lu2017fully, sun2020adashare, vandenhende2019branched}.

The main goal in multi-task learning is to improve individual tasks by focusing on task relatedness, which is non-trivial since the tasks might be learned with different learning rates or tasks, some tasks may be dominated by other tasks' poor learning, or interference between tasks gradients in backward propagation can impact on the generalization of model. Some gradient-based techniques have been proposed to solve the gradient conflict between tasks which mostly compare gradients of each pair of tasks \cite{sener2018multi, chen2018gradnorm, yu2020gradient}.

Training a good MTL model can be more difficult when the number of tasks grows, and improper sharing of information across unrelated tasks may lead to negative transfer. Accordingly, finding groups of tasks that can benefit from training together in an MTL setting is a promising way to avoid negative transferring and train a more accurate model that can perform better than simply training all tasks together \cite{standley2020tasks, fifty2021efficiently, kang2011learning}. The problem of deciding which tasks should be trained together recently has been tackled by human experts or algorithmic. Some MTL modeling approaches capture relationships among tasks by assuming that the task relationships are not known beforehand and can be learned directly from the data \cite{kang2011learning, jacob2008clustered, zhang2012convex}.

In \cite{jacob2008clustered} tasks are assumed to be clustered and parameters of tasks within a cluster lie close to each other in $ \ell2 $ norm sense and learn shared features with convex optimization. In \cite{zhang2012convex} tasks are assumed to share a common yet latent feature representation and learn shared features with convex optimization. In \cite{kang2011learning} tasks are assumed to form disjoint groups and that the tasks within each group lie in a low-dimensional subspace. Within each group, tasks share the same feature representation, whose parameters are learned jointly with the group assignment matrix using an alternating minimization scheme. However, a total disjointness between groups might not be the ideal way, as the tasks might still share some features that are helpful for prediction.



==> temp.tex <==
Multi-task learning (MTL) has been used successfully across all applications of machine learning, from natural language processing [Collobert and Weston, 2008] and speech recognition [Deng et al., 2013] to computer vision [Girshick, 2015] and drug discovery [Ramsundar et al., 2015].

In The function of TFs is to regulate expression of the correct number of genes in the body at the right time. TFs play important functions in many biological processes, such as gene transcription regulation, participation in developmental processes, and are closely related to many diseases. HM changes the binding environment of TFs to target sites by affecting the affinity between histone and DNA [9].

We assume that our data consists of $n$ “points” $x1,...,xn$ which can be arbitrary objects. We measure their pairwise similarities sij = s(xi,xj ) by some similarity function which is symmetric and nonnegative, and we denote the corresponding similarity matrix by $S = (s_{ij})_{i,j=1,...,n}$.

Given a dataset of $n p-dim$ points, $D = \{x_j\}^n_{j=1}$, the kmeans algorithm partitions the $n$ points into $k$ clusters, and represents each cluster by a center point. Let $C \in \mathbb{R}^{p×k}$ be a matrix whose columns comprise the $k$ cluster centers, i.e., $C = [c_1, c_2, \cdots , c_k]$. The k-means objective is to minimize the within-cluster squared distances:
